Improving Federated Aggregation with Deep Unfolding Networks

The performance of Federated learning (FL) is negatively affected by device differences and statistical characteristics between participating clients. To address this issue, we introduce a deep unfolding network (DUN)-based technique that learns adaptive weights that unbiasedly ameliorate the adverse impacts of heterogeneity. The proposed method demonstrates impressive accuracy and quality-aware aggregation. Furthermore, it evaluated the best-weighted normalization approach to define less computational power on the aggregation method. The numerical experiments in this study demonstrate the effectiveness of this approach and provide insights into the interpretability of the unbiased weights learned. By incorporating unbiased weights into the model, the proposed approach effectively addresses quality-aware aggregation under the heterogeneity of the participating clients and the FL environment. Codes and details are \href{https://github.com/shanikairoshi/Improved_DUN_basedFL_Aggregation}{here}.

==> templatex/gitinfo/post-checkout <==
#!/bin/sh
# Copyright 2015 Brent Longborough
# Part of gitinfo2 package Version 2
# Release 2.0.7 2015-11-22
# Please read gitinfo2.pdf for licencing and other details
# -----------------------------------------------------
# Post-{commit,checkout,merge} hook for the gitinfo2 package
#
# Get the first tag found in the history from the current HEAD
FIRSTTAG=$(git describe --tags --always --dirty='-*' 2>/dev/null)
# Get the first tag in history that looks like a Release
RELTAG=$(git describe --tags --long --always --dirty='-*' --match '[0-9]*.*' 2>/dev/null)
# Hoover up the metadata
git --no-pager log -1 --date=short --decorate=short \
    --pretty=format:"\usepackage[%
        shash={%h},
        lhash={%H},
        authname={%an},
        authemail={%ae},
        authsdate={%ad},
        authidate={%ai},
        authudate={%at},
        commname={%cn},
        commemail={%ce},
        commsdate={%cd},
        commidate={%ci},
        commudate={%ct},
        refnames={%d},
        firsttagdescribe={$FIRSTTAG},
        reltag={$RELTAG}
    ]{gitexinfo}" HEAD > .git/gitHeadInfo.gin

==> templatex/gitinfo/post-commit <==
#!/bin/sh
# Copyright 2015 Brent Longborough
# Part of gitinfo2 package Version 2
# Release 2.0.7 2015-11-22
# Please read gitinfo2.pdf for licencing and other details
# -----------------------------------------------------
# Post-{commit,checkout,merge} hook for the gitinfo2 package
#
# Get the first tag found in the history from the current HEAD
FIRSTTAG=$(git describe --tags --always --dirty='-*' 2>/dev/null)
# Get the first tag in history that looks like a Release
RELTAG=$(git describe --tags --long --always --dirty='-*' --match '[0-9]*.*' 2>/dev/null)
# Hoover up the metadata
git --no-pager log -1 --date=short --decorate=short \
    --pretty=format:"\usepackage[%
        shash={%h},
        lhash={%H},
        authname={%an},
        authemail={%ae},
        authsdate={%ad},
        authidate={%ai},
        authudate={%at},
        commname={%cn},
        commemail={%ce},
        commsdate={%cd},
        commidate={%ci},
        commudate={%ct},
        refnames={%d},
        firsttagdescribe={$FIRSTTAG},
        reltag={$RELTAG}
    ]{gitexinfo}" HEAD > .git/gitHeadInfo.gin

==> templatex/gitinfo/post-merge <==
#!/bin/sh
# Copyright 2015 Brent Longborough
# Part of gitinfo2 package Version 2
# Release 2.0.7 2015-11-22
# Please read gitinfo2.pdf for licencing and other details
# -----------------------------------------------------
# Post-{commit,checkout,merge} hook for the gitinfo2 package
#
# Get the first tag found in the history from the current HEAD
FIRSTTAG=$(git describe --tags --always --dirty='-*' 2>/dev/null)
# Get the first tag in history that looks like a Release
RELTAG=$(git describe --tags --long --always --dirty='-*' --match '[0-9]*.*' 2>/dev/null)
# Hoover up the metadata
git --no-pager log -1 --date=short --decorate=short \
    --pretty=format:"\usepackage[%
        shash={%h},
        lhash={%H},
        authname={%an},
        authemail={%ae},
        authsdate={%ad},
        authidate={%ai},
        authudate={%at},
        commname={%cn},
        commemail={%ce},
        commsdate={%cd},
        commidate={%ci},
        commudate={%ct},
        refnames={%d},
        firsttagdescribe={$FIRSTTAG},
        reltag={$RELTAG}
    ]{gitexinfo}" HEAD > .git/gitHeadInfo.gin
